Towards Instance-Optimality in Online PAC Reinforcement Learning

Several recent works have proposed instance-dependent upper bounds on the number of episodes needed to identify, with probability $1-\delta$, an $\varepsilon$-optimal policy in finite-horizon tabular Markov Decision Processes (MDPs). These upper bounds feature various complexity measures for the MDP, which are defined based on different notions of sub-optimality gaps. However, as of now, no lower bound has been established to assess the optimality of any of these complexity measures, except for the special case of MDPs with deterministic transitions. In this paper, we propose the first instance-dependent lower bound on the sample complexity required for the PAC identification of a near-optimal policy in any tabular episodic MDP. Additionally, we demonstrate that the sample complexity of the PEDEL algorithm of \cite{Wagenmaker22linearMDP} closely approaches this lower bound. Considering the intractability of PEDEL, we formulate an open question regarding the possibility of achieving our lower bound using a computationally-efficient algorithm.

==> sections/4.algorithm.tex <==
\section{Implicit eliminations for smaller computational and memory complexities}
While PEDEL nearly matches the lower bound of Theorem \ref{thm:general-lb-epsilon}, it does so at the cost of enumerating the set of all deterministic policies. Indeed, PEDEL proceeds in phases where at every phase $k\in \mathbb{N}$ it stores a set of \emph{active} policies $\Pi^k$ and a set of estimates $(\widehat{V}_1^{\pi,k})_{\pi \in \Pi^k}$ of their respective values. The set of active policies is initialized with the value $\Pi^0 = \PiD$ and then updated at the end of each phase by computing upper and lower confidence bounds on the value of every policy in $\Pi^k$ and removing the ones that are provably sub-optimal (i.e. the policies whose upper-confidence bound on their value if smaller than the maximum lower-confidence bound). PEDEL stops whenever $\Pi^k$ is reduced to a singleton or it has reached $\cO(\epsilon)$ precision in the estimation of the values $(V_1^\pi)_{\pi\in\Pi^k}$. This results in an exponential memory and computational complexity. Therefore one might ask whether we can achieve the same sample complexity but within polynomial time and space. We give a partially positive answer to this question by proposing EDIPE, a PAC RL algorithm for the case of known transitions and unknown reward distributions. This generalizes the setting of MDPs with deterministic transitions studied in \cite{tirinzoni2022NearIP}. \\
EDIPE relies on the idea of \emph{implicit policy eliminations} to rule out sub-optimal policies in a time-memory efficient manner. We now explain how this idea works. Instead of working with sets of policies, EDIPE defines a set of \emph{active state-action distributions} which is initialized with 

The pseudo code of EDIPE is detailed in Algorithm \ref{alg:EDIPE}.
\begin{algorithm}[!ht]
\caption{ EDIPE (Experimental Design with Implicit PoLicy Elimination) }\label{alg:EDIPE}
\begin{algorithmic}[1]
\STATE \textbf{Input:}  Precision $\epsilon$, Risk $\delta$, transition kernel $\{p_h(.|s,a)\}_{h\in[H], s\in \cS, a\in \cA}$
\STATE \textbf{Output:}  A policy $\widehat{\pi}$ that is $\epsilon$-optimal w.p larger than $1-\delta$
\STATE Define target function $c_h^0(s,a) = \log(3SAH/\delta)$ for all $(h,s,a)$
\STATE Execute $\textsc{CovGame}\big(c^0,\ \delta/5\big)$ to get dataset $\cD_{0}$ and number of episodes $d_{0}$ \hfill \textsc{// Burn-in phase}
\STATE Initialize episode count $t_0 \leftarrow d_0$ and statistics $n_h^{0}(s,a), \widehat{r}_h^{0}(s,a)$ using $\widetilde{\cD}_{0}$
\STATE Initialize the set of active distributions $\Omega^{0} \leftarrow \Omega$

\FOR{$k=1,\dots$}
\STATE \blue{\textsc{// Experimental design minimization, phase $k$}
\STATE  Solve experimental design problem (\ref{eq:ellipsoidal_design_problem}) to get its solution $\eta^k$ and value $E^\star_k$
\begin{align}\label{eq:ellipsoidal_design_problem}
    E^\star_k:=  \underset{\eta\in\Omega}{\min} \max_{\red{\rho\in \Omega^{k-1}} }\sum_{h,s,a} \frac{\rho_h(s,a)^2}{\eta_h(s,a)}
\end{align}

\STATE  Extract exploration policy $\pi^{k}$ by normalizing\footnote{i.e. $\pi^{k}_h(a|s) = \frac{\eta_h^k(s,a)}{\sum_{b\in\cA}\eta_h^k(s,b)}$ if $\sum_{b\in\cA}\eta_h^k(s,b) > 0$ and $\pi^{k}_h(a|s) = 1/A$ otherwise.} $\eta^k$

\STATE Play $\pi^{k}$ for $d_{k}  \leftarrow \left\lceil 2^{k+1} E^\star_k \right\rceil$ episodes and store them in dataset $\cD_{k}$
}

\STATE Update episode count $t_{k} \leftarrow t_{k-1}+ d_{k} $ and statistics $n_h^{k}(s,a), \widehat{r}_h^{k}(s,a)$ using  dataset $\cD_{k}$ \\ 
\vspace{0.2cm}
\red{\normalsize{\textsc{// implicit policy elimination}}}
 
\STATE Compute the maximum lower confidence bound by solving
$$\underline{V}_1^{k} := \sup_{\substack{\rho \in \Omega,\\ \textstyle{\sum\limits_{h,s,a} \frac{\rho_h(s,a)^2}{n_h^{k}(s,a)} \leq 2^{-k}}}} \rho^\top \widehat{r}^{k} - \sqrt{2^{2-k}H\beta^{bpi}(t_{k},\delta/3)} $$ 

\STATE Update the set of active state-action distributions 
$$\red{\Omega^{k}} \leftarrow \bigg\{\rho \in \Omega:\  \rho^\top \widehat{r}^{k} \geq   \underline{V}_1^{k}\ \textrm{and}\ 
\sum\limits_{h,s,a} \frac{\rho_h(s,a)^2}{n_h^{k}(s,a)} \leq 2^{-k} \bigg\}$$

\STATE \textbf{if} $\sqrt{2^{2-k}\beta^{bpi}(t_{k},\delta/3)} \leq \epsilon$  \textbf{then} \hfill \textsc{// Stopping condition}
\STATE \quad Compute any $\widehat{\rho}^\star \in \argmax_{\rho \in \Omega^{k}} \rho^\top \widehat{r}^{k}$ and extract the corresponding policy $\widehat{\pi}$

\STATE \quad \textbf{return} $\widehat{\pi}$
\STATE \textbf{end if}
%\red{\small{\textsc{// Add one linear constraint to set of active flows} }}
\ENDFOR
 %\hfill{\color{gray!60!black}\small\textsc{// Recommendation rule}}
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:EDIPE-complexity}
With probability at least $1-\delta$, the sample complexity of EDIPE satisfies 
    \begin{align*}
        \tau \leq \widetilde{\cO}\bigg( \big(H^2\log(1/\delta) + SAH^3\big)\underset{\eta\in\Omega}{\min}\max_{\pi\in\PiD}\sum_{h,s,a} \frac{p^{\pi}_h(s,a)^2}{\eta_h(s,a)\max(\epsilon, \Delta(\pi))^2} +\varphi^\star(\mathds{1}) SAH^2 (\log(3/\delta) + S) \bigg)
    \end{align*}
\end{theorem}

that eliminating policies can be performed in a time-memory efficient manner and that the bottleneck of combined statistical and computational efficiency lies in the sampling rule    

==> sections/4.all_empirical_algorithm.tex <==
\section{Improving upon the computational efficiency of PEDEL}

The pseudo code of E2DIPE is detailed in Algorithm \ref{alg:E2DIPE}.
\begin{algorithm}[!ht]
\caption{ E2DIPE (Ellipsoidal Experimental Design with Implicit PoLicy Elimination) }\label{alg:E2DIPE}
\begin{algorithmic}[1]
\STATE \textbf{Input:}  Precision $\epsilon$, Confidence $\delta$, transition kernel $\{p_h\}_{h\in[H]}$
\STATE \textbf{Output:}  A policy $\widehat{\pi}$ that is $\epsilon$-optimal w.p larger than $1-\delta$
\STATE Define target function $c_h^0(s,a) = 2\log(3SAH/\delta)$ for all $(h,s,a)$
\STATE Execute $\textsc{CovGame}\big(c^0,\ \delta/5\big)$ to get dataset $\cD_{0}$ and number of episodes $d_{0}$ \hfill \textsc{// Burn-in phase}
\STATE Initialize episode count $t_0 \leftarrow d_0$ and statistics $n_h^{0}(s,a), \widehat{r}_h^{0}(s,a), \widehat{p}_h^{0}(.|s,a)$ using $\widetilde{\cD}_{0}$
\STATE Initialize the set of active distributions $\Omega^{0} \leftarrow \Omega(\widehat{p}^0)$

\FOR{$k=1,\dots$}
\STATE \blue{\textsc{// Ellipsoidal design minimization, phase $k$}
\STATE  Solve Ellipsoidal design problem (\ref{eq:ellipsoidal_design_problem}) to get its solution $\eta^k$ and value $E^\star_k$
\begin{align}\label{eq:ellipsoidal_design_problem}
    E^\star_k:=  \underset{\eta\in\red{\Omega}}{\min} \max_{\rho\in \Omega^{k-1} }\sum_{h,s,a} \frac{\rho_h(s,a)^2}{\eta_h(s,a)}
\end{align}
\red{problem, we don't know the real omega when minimizing over $\eta$. thus $\eta^k$ is NOT  the state-action distribution associated with $\pi^{k}$ in the true MDP!!}
\STATE  Extract exploration policy $\pi^{k}$ by normalizing\footnote{i.e. $\pi^{k}_h(a|s) = \frac{\eta_h^k(s,a)}{\sum_{b\in\cA}\eta_h^k(s,b)}$ if $\sum_{b\in\cA}\eta_h^k(s,b) > 0$ and $\pi^{k}_h(a|s) = 1/A$ otherwise.} $\eta^k$

\STATE Play $\pi^{k}$ for $T_{k,1}  \leftarrow \left\lceil 2^k E^\star_k \right\rceil$ episodes and store them in dataset $\cD_{k,1}$
}\\ \vspace{0.2cm}
\normalsize{\textsc{// Ensuring empirical ellipsoid concentrates around true ellipsoid}}

\STATE $(\cD_{k,2}, T_{k,2}) \leftarrow \textsc{EnhanceMinCount}(k, \delta)$

\STATE Update episode count $t_{k} \leftarrow t_{k-1}+ T_{k,1} + T_{k,2}$ and statistics $n_h^{k}(s,a), \widehat{r}_h^{k}(s,a), \widehat{p}_h^{k}(.|s,a)$ using  dataset $\cD_{k,1} \cup \cD_{k,2}$ \\ 
\vspace{0.2cm}
\red{\normalsize{\textsc{// implicit policy elimination}}}
 
\STATE Compute the lower confidence bound 
$$\underline{V}_1^{k} := \sup_{\substack{\widehat{\rho} \in \Omega(\widehat{p}^{k}),\\ \textstyle{\sum\limits_{h,s,a} \frac{\widehat{\rho}_h(s,a)^2}{n_h^{k}(s,a)} \leq 2^{-k}}}} \widehat{\rho}^\top \widehat{r}^{k} - \sqrt{2^{2-k}H\beta^{bpi}(t_{k},\delta/3)} $$ 

\STATE Update the set of active state-action distributions 
$$\Omega^{k} \leftarrow \bigg\{\rho \in \Omega(\widehat{p}^k):\  \rho^\top \widehat{r}^{k} \geq   \underline{V}_1^{k}\ \textrm{and}\ 
\sum\limits_{h,s,a} \frac{\widehat{\rho}_h(s,a)^2}{n_h^{k}(s,a)} \leq 2^{-k} \bigg\}$$

\STATE \textbf{if} $\sqrt{2^{1-k}\beta^{bpi}(t_{k},\delta/2)} \leq \epsilon$  \textbf{then} \hfill \textsc{// Stopping condition}
\STATE \quad Compute any $\rho^\star \in \argmax_{\rho \in \Omega^{k}} \rho^\top \widehat{r}^{k}$ and extract the corresponding policy $\widehat{\pi}$

\STATE \quad \textbf{return} $\widehat{\pi}$
\STATE \textbf{end if}
%\red{\small{\textsc{// Add one linear constraint to set of active flows} }}
\ENDFOR
 %\hfill{\color{gray!60!black}\small\textsc{// Recommendation rule}}
\end{algorithmic}
\end{algorithm}

\subsection{Sampling rule}

\subsubsection{EnhanceMinCount subroutine}

\begin{algorithm}[ht]
    \caption{EnhanceMinCount}\label{alg:enhance-min-count}
    \begin{algorithmic}[1]
    \STATE \textbf{Input:}  Phase number $k$,
    \STATE \textbf{Output:} A dataset $\cD$ of $d \leq x_k$ episodes satisfying $ n_h(s,a; \cD) \geq c_h^k(s,a)$ for all $(h,s,a)$
    \STATE Solve $x_k := \min\bigg\{x>0:\ x\geq SAH\beta^{bpi}\big(t_{k-1}+ T_{k,1}+x, \delta/2 \big) \bigg\}$

    \STATE  Compute targets $c_h^{k}(s,a) := \sqrt{2^{k}\beta^{bpi}(t_{k-1}+ T_{k,1} + x_k,\delta/2) }$ for all $(h,s,a)$

    \STATE Execute $\textsc{CovGame}\big(c^{k},\ \delta/6(k+1)^2 \big)$ to get dataset $\widetilde{\cD}_{k,2}$ and number of episodes $\widetilde{T}_{k,2}$

    \STATE \textbf{if} $\widetilde{T}_{k,2} > x_k $ \textbf{then} 
    \STATE \quad Run $\textsc{PruneDataset}(\widetilde{\cD}_{k,2}, c^k)$ to get \textit{effective} dataset $\cD_{k,2}$ and \textit{effective phase length} $T_{k,2}$
    \STATE \textbf{else}
    \STATE \quad Set  $T_{k,2} \leftarrow \widetilde{T}_{k,2}$ and $\cD_{k,2} \leftarrow \widetilde{\cD}_{k,2}$
    \STATE \textbf{end if}
    \STATE \textbf{return} $(\cD_{k,2}, T_{k,2})$
    
    \end{algorithmic}
\end{algorithm}

\subsubsection{PruneDataset subroutine}

\begin{algorithm}[ht]
    \caption{PruneDataset}\label{alg:prune-episodes}
    \begin{algorithmic}[1]
    \STATE \textbf{Input:}  Target counts $c$, Dataset $\widetilde{\cD}$ such that $n_h(s,a; \widetilde{\cD}) \geq c_h(s,a)$ for all $(h,s,a)$ 
    \STATE \textbf{Output:} A dataset $\cD$ of $d \leq SAH 2^k$ episodes satisfying $n_h(s,a; \cD) \geq c_h(s,a)$ for all $(h,s,a)$
    \STATE Initialize dataset $\cD \leftarrow \emptyset$, episode number $d\leftarrow 0$ and dataset-counts $n_h(s,a;\cD) \leftarrow 0$ for all $(h,s,a)$
    
    \FOR{episode $e = (s_\ell^e, a_\ell^e, R_\ell^e)_{1\leq \ell\leq H}$ in $\widetilde{\cD}$}
    \STATE \textbf{if} $\exists \ell \in [H]$ such that $n_\ell(s_\ell^e, a_\ell^e; \cD) < c_\ell(s_\ell^e, a_\ell^e)$ \textbf{then} 
    \STATE \quad Update dataset-counts $n_h(s_h^e,a_h^e;\cD) \leftarrow n_h(s_h^e,a_h^e;\cD) +1 $ for all $h\in [H]$
    \STATE \quad Update dataset $\cD \leftarrow \cD \cup \{e\}$ and episode number $d \leftarrow d+1$
    
    \STATE \quad \textbf{if} $n_h(s,a; \cD) \geq c_h(s,a)$ for all $(h,s,a)$ \textbf{then}
    \STATE \quad \quad \textbf{return} $(\cD, d)$
    \STATE  \quad \textbf{end if}
    \STATE \textbf{end if}
    \ENDFOR
    \end{algorithmic}
\end{algorithm}

\subsection{Good event}
We define the events
\begin{align*}
    \cE_p &:= \bigg(\forall k \in \mathbb{N}^\star\ \forall \pi \in \PiS\ \forall \widetilde{r}\in[0,1]^{SAH},\\
    &\quad\quad\quad  \Big|\sum_{h,s,a} \big(\widehat{p}_h^{\pi,k}(s,a)- p_h^{\pi}(s,a)\big) \widetilde{r}_h(s,a) \Big| \leq \sqrt{\beta^{bpi}(t_k,\delta/3)\min\bigg(\sum_{h,s,a}\frac{p_h^{\pi}(s,a)^2}{n_h^k(s,a)},\ \sum_{h,s,a}\frac{\widehat{p}_h^{\pi,k}(s,a)^2}{n_h^k(s,a)}\bigg)} \bigg)\\
    \cE_{pr} &:= \bigg(\forall k \in \mathbb{N}^\star\ \forall \pi \in \PiS,\\
    &\quad\quad\quad  \bigg|\sum_{h,s,a} \Big[\widehat{p}_h^{\pi,k}(s,a)\widehat{r}_h^{k}(s,a) - p_h^{\pi}(s,a) r_h(s,a)\Big] \bigg| \leq \sqrt{\beta^{bpi}(t_k,\delta/3)\min\bigg(\sum_{h,s,a}\frac{p_h^{\pi}(s,a)^2}{n_h^k(s,a)},\ \sum_{h,s,a}\frac{\widehat{p}_h^{\pi,k}(s,a)^2}{n_h^k(s,a)}\bigg)} \bigg)\\
    \cE_{cnts} &:= \bigg(\forall t\in\mathbb{N}_{>0}\ \forall (h,s,a),\  n_h^t(s,a) \geq \frac{1}{2}\overline{n}_h^t(s,a) - \log(3SAH/\delta) \bigg)\\
    \cE_{cov} &:= \bigg(\forall k\in \mathbb{N},\ \textrm{CovGame run with inputs $(c^{k}, \delta/6(k+1)^2)$ terminates after at most}\\
    & 64 m_k \varphi^\star(c^{k}) + \widetilde{\cO}\big(m_k \varphi^\star(\mathds{1}) SAH^2 (\log(6(k+1)^2/\delta) + S) \big)\ \textrm{episodes and returns a dataset $\cD_k$ }\\
    &\textrm{such that for all } (h,s,a)\in \widehat{\cX}, n_h(s,a;\cD_k)\geq c^{k}_h(s,a) \bigg),
\end{align*}
where $m_k = \log_2\big(\frac{\max_{s,a,h} c_h^{k}(s,a)}{\min_{s,a,h} c_h^{k}(s,a) \vee 1}\big) \vee 1$ and $\beta^{bpi}$ is defined in appendix \ref{sec:app-concentration-RFE}. Then our good event is defined as the intersection 
\begin{align*}
    \cE_{good} :=  \cE_{p} \cap \cE_{pr} \cap \cE_{cnts} \cap \cE_{cov}.
\end{align*}

\subsection{Optimal policies are never eliminated}
\begin{lemma}
    Under the good event, for all policies $\pi^\star \in \Pi^\star$ and all phases $k\geq 0$, it holds that at the end of phase $k$
    \begin{align*}
        \widehat{p}^{\pi^\star, k} \in \Omega^k\ \textrm{and}\ \sum_{h,s,a}\frac{p_h^{\pi}(s,a)^2}{n_h^k(s,a)}\leq 2^{-k}.
    \end{align*}
\end{lemma}
\begin{proof}
We fix an optimal policy $\pi^\star$ and prove the statement by induction. For $k=0$ the fact that $\widehat{p}^{\pi^\star, 0} \in \Omega^0$ is trivial, since $\Omega^0 = \Omega(\widehat{p}^0)$ consists of all state-action distributions that are valid under the transition kernel $\widehat{p}^0$. On the other hand,
\begin{align*}
    \sum_{h,s,a}\frac{p_h^{\pi^\star}(s,a)^2}{n_h^0(s,a)} &\leq  \sum_{h,s,a}\frac{p_h^{\pi}(s,a)}{H+2\log(3\delta/SAH)} \leq 2^{-0},
\end{align*}
where we used that $n_h^0(s,a) \geq c_h^0(s,a) = H+2\log(3\delta/SAH)$. Now suppose that the property holds at the end of phase $k-1$. We first show that $\max(\sum_{h,s,a} \frac{p_h^{\pi^\star}(s,a)^2}{n_h^{k}(s,a)},\ \sum_{h,s,a} \frac{\widehat{p}_h^{\pi^\star, k}(s,a)^2}{n_h^{k}(s,a)}) \leq 2^{-k}$. To that end, let us write 
\begin{align*}
    \bigg|\sum_{h,s,a} \frac{\widehat{p}_h^{\pi^\star, k-1}(s,a)^2}{n_h^{k}(s,a)}  - \sum_{h,s,a} \frac{p_h^{\pi^\star}(s,a)^2}{n_h^{k}(s,a)} \bigg| &= \bigg|\sum_{h,s,a} \Big(\widehat{p}_h^{\pi^\star, k-1}(s,a) - p_h^{\pi^\star}(s,a) \Big) \frac{\widehat{p}_h^{\pi^\star, k-1}(s,a) + p_h^{\pi^\star}(s,a)}{n_h^{k}(s,a)} \bigg| \\
    &\stackrel{(a)}{\leq} \frac{2}{\min_{h,s,a} n_h^{k}(s,a)}\sqrt{\beta^{bpi}(t_{k-1},\delta/3)\sum_{h,s,a}\frac{p_h^{\pi^\star}(s,a)^2}{n_h^{k-1}(s,a)}}\\
    &\stackrel{(b)}{\leq} 2\sqrt{\frac{2^{-k}}{\beta^{bpi}(t_{k-1},\delta/3)}} \sqrt{\beta^{bpi}(t_{k-1},\delta/3) 2^{1-k}} \leq  2^{-(k+1)},
\end{align*}
where (a) used the concentration event $\cE_p$ for the reward vector $\widetilde{r} = \bigg[\frac{\big(\widehat{p}_h^{\pi^\star, k-1}(s,a) + p_h^{\pi^\star}(s,a)\big)\min_{\ell,s',a'}n_\ell^{k}(s',a')}{2 n_h^{k}(s,a)} \bigg]_{h,s,a}$ and (b) used. Similarly, we have
\begin{align*}
    \bigg|\sum_{h,s,a} \frac{\widehat{p}_h^{\pi^\star, k-1}(s,a)^2}{n_h^{k}(s,a)}  - \sum_{h,s,a} \frac{\widehat{p}_h^{\pi^\star, k}(s,a)^2}{n_h^{k}(s,a)} \bigg| &\leq \bigg|\sum_{h,s,a} \frac{\widehat{p}_h^{\pi^\star, k-1}(s,a)^2}{n_h^{k}(s,a)}  - \sum_{h,s,a} \frac{p_h^{\pi^\star}(s,a)^2}{n_h^{k}(s,a)} \bigg| + \bigg| \sum_{h,s,a} \frac{p_h^{\pi^\star}(s,a)^2}{n_h^{k}(s,a)} - \sum_{h,s,a} \frac{\widehat{p}_h^{\pi^\star, k}(s,a)^2}{n_h^{k}(s,a)} \bigg|  \\
    &\leq \frac{2}{\min_{h,s,a} n_h^{k}(s,a)}\sqrt{\beta^{bpi}(t_{k-1},\delta/3)\sum_{h,s,a}\frac{p_h^{\pi^\star}(s,a)^2}{n_h^{k-1}(s,a)}}\\
    &\quad + \frac{2}{\min_{h,s,a} n_h^{k}(s,a)}\sqrt{\beta^{bpi}(t_{k},\delta/3)\sum_{h,s,a}\frac{p_h^{\pi^\star}(s,a)^2}{n_h^{k}(s,a)}}\\
    &\stackrel{(a)}{\leq} \frac{4}{\min_{h,s,a} n_h^{k}(s,a)}\sqrt{\beta^{bpi}(t_{k},\delta/3)\sum_{h,s,a}\frac{p_h^{\pi^\star}(s,a)^2}{n_h^{k-1}(s,a)}}\\
    &\leq 4\sqrt{\frac{2^{-k}}{\beta^{bpi}(t_{k-1},\delta/3)}} \sqrt{\beta^{bpi}(t_{k},\delta/3) 2^{1-k}} \leq 2^{-(k+1)},
\end{align*}
where (a) used that $n_h^{k}(s,a) \ge n_h^{k-1}(s,a)$ for all $(h,s,a)$ and that $t \mapsto \beta^{bpi}(t,\delta)$ is non-decreasing.
Let $\widetilde{\rho} \in \argmax_{\rho \in \Omega^{k-1}} \rho^\top \widehat{r}^{k}$ and consider any policy $\widetilde{\pi}$ whose state-action distribution is $\widetilde{\rho}$. Under the good event we have,
\begin{align*}
    (p^{\pi^\epsilon})^\top \widehat{r}^{k} - \underline{V}_1^{k} +\epsilon &\stackrel{(a)}{=} \widehat{V}_1^{\pi^\epsilon, t_k} - \widehat{V}_1^{\widetilde{\pi}, t_k} + \sqrt{2^{1-k}\beta^{r}(t_{k},\delta/2)} + \epsilon\\
    &\stackrel{(b)}{\geq} \widehat{V}_1^{\pi^\epsilon, t_k} - \widehat{V}_1^{\widetilde{\pi}, t_k} + \sqrt{\beta^r(t_k,\delta/2) \sum_{h,s,a} \frac{\big(p_h^{\pi^\epsilon}(s,a)-p_h^{\widetilde{\pi}}(s,a)\big)^2}{n_h^{t_k}(s,a)}} + \epsilon\\
    &\stackrel{(c)}{\geq} V_1^{\pi^\epsilon} - V_1^{\widetilde{\pi}} + \epsilon\\
    &\geq 0,
\end{align*}
where (a) uses the definition of $\underline{V}_1^{k}$ and $\widetilde{\pi}$ while (b) and (c) use Lemmas \ref{lem:harmonic-proportional-coverage} and \ref{lem:global-concentration-comparison} respectively. Therefore we just proved that $p^{\pi^\epsilon} \in \{\rho \in \mathbb{R}_{+}^{SAH}:\  \rho^\top \widehat{r}^{k} \geq   \underline{V}_1^{k} - \epsilon\ \}$, and consequently $p^{\pi^\epsilon} \in \Omega^k$.
\end{proof}
